Ring-Zero: Scaling Zero RL to a Trillion Parameters for Emergent Reasoning

Reinforcement learning with verifiable rewards without human-annotated data, often referred to as zero RL, has emerged as a powerful paradigm for eliciting chain-of-thought reasoning. However, due to computational constraints, existing studies are largely restricted to small models, leaving the training dynamics and emergent capabilities at a large scale unexplored. To meaningfully explore this frontier, we aim to elicit high-quality reasoning behaviors from the model. However, we find that naive scaling often suffers from poor readability, token redundancy, and a lack of adaptive reasoning depth. To address these challenges, we present a stable and efficient training pipeline, incorporating algorithmic and system optimizations such as clipped importance sampling, training-inference ratio correction, and mixed-precision control. Our experiments offer three key findings that validate the "bitter lesson" of scaling: (1) scaling to 1T parameters significantly enhances sample efficiency and performance ceilings; (2) the training process progresses sequentially through an initial discovery phase followed by a sharpening phase; and (3) the model spontaneously develops advanced cognitive behaviors, including anthropomorphism, structured formatting, self-verification, parallel reasoning, and context anxiety, rendering hand-crafted heuristics redundant. Evaluated on seven mathematical benchmarks, Ring-2.5-1T-Zero achieves competitive performance. Additionally, to assess CoT quality beyond final-answer correctness, we propose a structured evaluation framework across three dimensions: comprehensibility, reproducibility, and efficiency, where our model demonstrates clear advantages in producing structured and concise reasoning traces. By sharing our observed emergent phenomena, we hope to provide the community with deeper insights into scaling behaviors, particularly at the 1-trillion scale.

==> case/all_cases.tex <==
% Case study: Model responses to the sequence problem
% "Consider a sequence of positive integers with a total sum of 2019
%  such that no number and no sum of a set of consecutive numbers is equal to 40.
%  What is the greatest possible length of such a sequence?"
%
% Required package: tcolorbox (with breakable library)
% \usepackage[breakable]{tcolorbox}
%
% Box definition:
% \newtcolorbox{promptbox}[2][Prompt]{%
%   breakable, colback=#2!6!white, arc=5pt, boxrule=0.5pt,
%   fonttitle=\bfseries, title=#1, colframe=#2!70!black,
%   width=0.98\linewidth, left skip=0.01\linewidth, right skip=0.01\linewidth,
% }

\section{Comparison of Our CoT with Other Models}

In this section, we compare the Chain-of-Thought (CoT) reasoning traces generated by our model with those produced by other state-of-the-art models.

\begin{promptbox}[Question]{black}
Consider a sequence of positive integers with a total sum of $2019$ such that no number and no sum of a set of consecutive numbers is equal to $40$. What is the greatest possible length of such a sequence?

Please reason step by step, and put your final answer within $\boxed{}$.
\end{promptbox}

\vspace{0.5em}
\input{gpt-5.5.tex}

\vspace{0.5em}
\input{claude-opus-4.7.tex}

\vspace{0.5em}
\input{ring-zero.tex}

\vspace{0.5em}
\input{deepseek-v4-pro.tex}

\vspace{0.5em}
\input{gemini-3.1-pro.tex}

\vspace{0.5em}
\input{doubao-2.0.tex}

\vspace{0.5em}
\input{kimi-k2.6.tex}

\vspace{0.5em}
\input{qwen3.5.tex}

\vspace{0.5em}
\input{glm-5.1.tex}

\vspace{0.5em}
\input{minimax-2.7.tex}


==> tables/experimental_setup.tex <==
\begin{table}[t]
\centering
\caption{Stage-specific hyperparameter configurations.}
\label{tab:hyper}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Configuration} & \textbf{Stage I} & \textbf{Stage II} & \textbf{Stage III} \\
\midrule
Loss Reduction & Token & Sample & Sample \\
KL Coefficient ($\beta$) & $1 \times 10^{-4}$ & $0$ & $0$ \\
KL Type & K3 & K1 & -- \\
Max Response Length & 4k $\rightarrow$ 16k & 16k & 4k / 16k / 64k \\
Global Batch Size & 7680 & 7680 & 7680 \\
Sequence Length & 16384 & 16384 & 4096 / 16384 / 65536 \\
Training Steps & $\sim$1100 & $\sim$1100 & $\sim$1100 \\
Response Tiers & Single & Single & Low / Mid / High \\
\bottomrule
\end{tabular}
}
\end{table}
